Multimodal Coreference Resolution for Chinese Social Media Dialogues: Dataset and Benchmark Approach

Multimodal coreference resolution (MCR) aims to identify mentions referring to the same entity across different modalities, such as text and visuals, and is essential for understanding multimodal content. In the era of rapidly growing mutimodal content and social media, MCR is particularly crucial for interpreting user interactions and bridging text-visual references to improve communication and personalization. However, MCR research for real-world dialogues remains unexplored due to the lack of sufficient data resources. To address this gap, we introduce TikTalkCoref, the first Chinese multimodal coreference dataset for social media in real-world scenarios, derived from the popular Douyin short-video platform. This dataset pairs short videos with corresponding textual dialogues from user comments and includes manually annotated coreference clusters for both person mentions in the text and the coreferential person head regions in the corresponding video frames. We also present an effective benchmark approach for MCR, focusing on the celebrity domain, and conduct extensive experiments on our dataset, providing reliable benchmark results for this newly constructed dataset. We will release the TikTalkCoref dataset to facilitate future research on MCR for real-world social media dialogues.

==> ethical_considerations.tex <==
\section{Ethical Considerations}
Our TikTalkCoref dataset is built based on the TikTalk dataset \cite{Lin-2023-Tiktalk}. We have submitted a application form for usage rights to the authors and obtained permission. We will make our TiktalkCoref dataset publicly available in the near future. The release of the dataset will fully comply with the fair use principle in copyright law. 

For the annotation payment, we compensate all annotators based on their annotation time and quality. The average salary is 20 RMB per hour, which is a fair and reasonable wage level in China.



==> response.tex <==

\noindent Dear Reviewers,

We are sending herewith a revised manuscript ``Multimodal Coreference Resolution for Chinese Social Media Dialogues: Dataset and Benchmark Approach'' that we would like to submit to ACL ARR 2025 February. 
% Our previous URL is \url{https://openreview.net/forum?id=22fxMwp3rq#discussion}, 
% with an average overall assessments in the last ARR cycle of 3. 
We really appreciate the substantial comments and suggestions from the reviewers. We have carefully studied all the comments and made the following major modifications in the current submission. 

\section*{Revision Summary}

% \subsection*{Add more experiments and analysis:}
\noindent \textbf{Add more information about the TikTalkCoref dataset and analysis:}

• Added the size comparison of each dataset in Table \ref{tab:dataset_comparison}. (Suggested by Reviewer jhCa)

• Added statistical significance tests in Section \ref{sec:Experiments}. (Suggested by Reviewer 8sjx)

• Added statistical information on dialogues mentioning celebrities in Table \ref{tab:data basic statistics}. (Suggested by Reviewer jhCa)

• Added statistical information on the gender, age, and occupation of  persons in the TikTalkCoref dataset in Appendix \ref{appendix:key information}. (Suggested by Reviewer jhCa)%+跳转链接


\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Improve the clarity:}

% • Added a clear explanation for why our task is limited to the celebrity domain in Section \ref{sec:Introduction}. (jhCa, b4eS)
• Added a clear explanation of task domain in Abstract and Section \ref{sec:Introduction}. (Suggested by Reviewer jhCa, b4eS)

• Revised the statement about ``capturing the complexity and diversity of multimodal information interaction in the real world'' in lines 58-61 and lines 126-129. (Suggested by Reviewer b4eS)

• Added a clear definition of ``cross-modal coreference relationships'' in Section \ref{sec:Introduction}. (Suggested by Reviewer b4eS)

• Added a clear explanation of the high-quality data filtering criteria in Section \ref{sec:Data Selection}. (Suggested by Reviewer b4eS)

• Added a clear explanation of the celebrity identification criteria in Section \ref{sec:Annotation Guidelines}. (Suggested by Reviewer b4eS)

• Use the average MUC score \cite{pradhan-etal-2012-conll} as our inter-annotator agreement metric in Section \ref{sec:Data Statistics and Analysis}. (Suggested by Reviewer 8sjx)

• Added the reasons why we use e2e-coref as the baseline and why we choose current baselines and why we use non-celebrity data during training in Section \ref{sec:Experimental Settings}. (Suggested by Reviewer jhCa)


• Added detailed explanation for evaluation indicators in Appendix \ref{appendix:evaluation indicators}. (Suggested by Reviewer wRGo)



\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Rectified typos:} 

• Corrected typos in the Figure \ref{fig:the overview of our pipeline}.

\vspace{0.5em}  % 调整段落间距
\textbf{To facilitate the next ARR cycle review, we have attached an annotated manuscript in the end of this response PDF, in which our major modifications are \textcolor{red}{highlighted in red color}. Reviewers can click on the hyperlinks in Response to directly jump to the corresponding revised sections.} In the following, we give point-to-point responses regarding to comments from our reviewers in the previous submission.

% \section*{General Response}
% \textbf{The General Concern 1:} \textit{The data scale and diversity of our TikTalkCoref dataset.}

% \vspace{0.5em}  % 调整段落间距
% \noindent \textbf{Our Response:} 
% % We would explain the reasons behind the small scale and limited diversity of our dataset. 
% % The TikTalkCoref dataset is relatively small in scale and limited in diversity, primarily due to the labor-intensive and time-consuming nature of aligning multimodal coreference data. Each dialogue involves complex textual coreference chains that must be accurately linked to head images of individuals in videos. 

% % Our focus on multimodal coreference resolution in dialogue scenarios let us to deliberately select tightly controlled contexts and concentrate on the ``celebrity'' category to ensure high-quality annotations and reliable evaluations. While this approach has resulted in a high-quality benchmark dataset, it has also constrained the dataset's size and diversity. 
% The annotation of multimodal coreference resolution is an extremely labor-intensive and time-consuming task. To ensure data quality, we have implemented strict controls over the annotation process. To date, we have annotated a total of 1,012 dialogues and videos.

% Although our dataset TikTalkCoref may not be large in scale, as the first real-world Chinese multimodal coreference resolution dataset, it holds unique and pioneering significance, particularly for cross-modal alignment and coreference resolution in Chinese. We believe TikTalkCoref will provide essential data support for research in Chinese multimodal coreference resolution.

% In future work, we plan to expand the dataset by incorporating data from more diverse sources and adding more object categories to improve generalization. Additionally, we will explore methods for implementing multimodal coreference resolution in low-resource conditions.

% \vspace{1em}  % 调整段落间距
% \noindent \textbf{The General Concern 2:} \textit{The reason why only celebrity data in TikTalkCoref is used when training the benchmark model.}

% \vspace{0.5em}  % 调整段落间距
% \noindent \textbf{Our Response:} When performing cross-modal coreference alignment, we aim to use knowledge bases of persons to improve the alignment. However, publicly available knowledge bases typically only cover celebrities. To simplify the task and achieve better alignment, we currently focus on multimodal coreference resolution for celebrities. For a broader range of persons, we plan to explore this in future work.

% \vspace{1em}  % 调整段落间距
% \noindent \textbf{The General Concern 3:} \textit{More comparison with existing multimodal coreference resolution models.}

% \vspace{0.5em}  % 调整段落间距
% \noindent \textbf{Our Response:} 
% We have compared two models in the cross-modal coreference alignment module: CN-CLIP and R2D2. Both models have been pre-trained on large-scale Chinese datasets and have demonstrated strong performance in Chinese text-image matching and visual information extraction. We also attempted to compare them with existing multimodal coreference resolution models; however, most of these models are trained on English data, and their methods and pre-trained models are not optimized for Chinese. Additionally, our dataset does not provide sufficient data to support effective fine-tuning of English-based models. Therefore, we only used CN-CLIP and R2D2 as baseline models. 

% In the future, we will explore how to perform multimodal coreference resolution under low-resource conditions and build a more effective and robust model.
% % Most existing multimodal coreference resolution models are trained on English data, and their methods and pretrained models are not optimized for Chinese. Additionally, due to the relatively small size of our dataset, we are unable to provide enough data to effectively fine-tune English models. Therefore, using existing multimodal coreference resolution models as comparison baselines for our task is quite challenging, and the results may not be ideal, particularly in the case of scarce data resources. In future work, we will explore how to perform transfer learning under low-resource conditions to obtain more robust comparison baseline results.

% % Ultimately, we decided to build a pipeline suitable for Chinese multimodal coreference resolution and selected CN-CLIP and R2D2 as the baseline models. Both of these models have been pretrained on large amounts of Chinese data and have demonstrated strong performance in Chinese text-image matching and visual information extraction. We believe they can serve as benchmarks to evaluate the effectiveness of our approach.


\vspace{1em}  % 调整段落间距
\section*{Response to Meta Reviewer 8sjx}
\textbf{Question 1:} \textit{The TikTalkCoref dataset has the following limitations: (a) the dataset is based on a single social media platform, (b) uses a single language (Chinese), (c) is limited to the category ``People'', (d) does not come across as a representative sample (filtering criteria, focus on celebrities etc.), (e) is of a small scale.} 

\vspace{0.5em}  % 调整段落间距

\noindent \textbf{Our Response:} 

\textbf{• The data scale and diversity of our TikTalkCoref dataset:}
The annotation of multimodal coreference resolution is an extremely labor-intensive and time-consuming task, so that we have invested significant effort into the annotation process. To ensure data quality, we have implemented strict controls on the data source and annotation process. To date, we have annotated a total of 1,012 dialogues and videos. Although our dataset TikTalkCoref may not be large in scale, as the first real-world Chinese multimodal coreference resolution dataset, it holds unique and pioneering significance, particularly for cross-modal alignment and coreference resolution in Chinese. 
In future work, we plan to expand the dataset by incorporating data from more diverse sources and adding more object categories to improve generalization. 

\textbf{• The reason why only celebrity data in TikTalkCoref is used:}
When performing cross-modal coreference alignment, we aim to use knowledge bases of persons to improve the alignment. However, publicly available knowledge bases typically only cover celebrities. To simplify the task and achieve better alignment, we currently focus on multimodal coreference resolution for celebrities. In future work, we plan to explore broader groups of persons.


% Our dataset is small and limited in diversity due to the labor-intensive nature of aligning multimodal data and the focus on tightly controlled contexts for high-quality annotations. We are actively working to address these issues, and in future work, we will expand the dataset size and increase its diversity. For more detailed information, please refer to the \textbf{General Response}.
% Regarding the limitations in (a), (c), and (e), the reason for the relatively small scale and low diversity of the TikTalkCoref dataset is that multimodal coreference annotation is highly labor-intensive, requiring annotators to invest significant time and effort to ensure high-quality annotations and consistency in multimodal coreference. 

% Regarding the limitations in (b), the lack of multimodal coreference resolution work in the Chinese language domain has also led us to focus more on the annotation of multimodal coreference data in Chinese.

% Regarding the limitations in (d), our intentional focus on a single object category—"celebrities"—is due to the fact that existing knowledge bases typically only include celebrities, making it difficult to obtain image-text pairs and knowledge for non-celebrities to train our model. To ensure reliable annotations and evaluations, we have limited the task to the celebrity domain. 

% Of course, we acknowledge the importance of expanding the dataset’s scale and diversity for broader generalization, and we plan to introduce data from multiple sources and other object categories in future work.

\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 2:} \textit{The paper should add more compelling baseline comparisons and contextualise the results with what has been reported in the literature as state-of-the-art results.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have compared two models in the cross-modal coreference alignment module: CN-CLIP \cite{chineseclip} and R2D2 \cite{xie-2023-ccmb}. Both models have been pre-trained on large-scale Chinese datasets and have demonstrated strong performance in Chinese text-image matching and visual information extraction. We also attempted to compare them with existing multimodal coreference resolution models; however, most of these models are trained on English data, and their methods and pre-trained models are not optimized for Chinese. Additionally, our dataset does not provide sufficient data to support effective fine-tuning of English-based models. Therefore, we only used CN-CLIP and R2D2 as baselines. In future work, we will explore methods for implementing multimodal coreference resolution in low-resource conditions.
% Due to language and data scale issues, existing multimodal coreference resolution models may be difficult to apply to our task. We are working on addressing this problem and will explore how to perform transfer learning under low-resource conditions in order to obtain more robust comparison baseline results. The detailed information is shown in the \textbf{General Response}.

\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 3:} \textit{Throughout the paper terminology such as ``significant'' and ``outperform'' is being used without reference to suitable statistical significance tests.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have added the significance tests using Dan Bikel's randomized parsing evaluation comparator \cite{noreen-1989-test} in Section \ref{sec:Experiments}, with a significance level set to 0.001. The results demonstrate that there is a significant difference between the two sets of benchmark results in both the textual coreference resolution and cross-modal alignment experiments.

\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 4:} \textit{It is suggested that the inter-annotator agreement figures are being strengthened by adopting commonly used metrics as they provide more insight.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} To assess inter-annotator agreement more accurately and objectively, following common approaches \cite{pradhan-etal-2012-conll}, we use the average MUC score between the annotations of two annotators as the evaluation metric, obtaining the MUC score of 78.19, which is explained in Section \ref{sec:Data Statistics and Analysis}. 
% After our research, we find that the commonly used metric Kappa agreement, as well as the consistency metric MUC \cite{pradhan-etal-2012-conll}, are not suitable for our task. 

% In coreference resolution, the number of categories (i.e., clusters) for each instance is dynamic, and the number of elements (i.e., mentions) within each cluster is also uncertain. Since the Kappa agreement is typically used for classification tasks with fixed numbers of categories, this makes it challenging to apply the Kappa agreement to our task. At the same time, since our dataset contains a large number of singleton clusters, the MUC metric, which focuses on matching coreference links between mentions, is also difficult to accurately reflect our annotation agreement.

% Therefore, based on the Jaccard coefficient \cite{Jaccard1901}, we have designed two agreement metrics suitable for our task, which can more comprehensively assess annotation agreement from both the cluster and mention dimensions.


\vspace{1em}
\section*{Response to Reviewer jhCa}
\textbf{Question 1:} \textit{The created dataset TikTalkCoref is relatively small in scale and not diverse enough.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have devoted substantial effort to data annotation, resulting in a collection of 1,012 annotated dialogues. 
% These data will advance research in Chinese multimodal coreference resolution.
In the future, we will expand the dataset' s scale and diversity.
For details, please refer to \textbf{Response to Meta Reviewer}.

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 2:} \textit{Missing key information of the dataset and comparison of its size with other datasets.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have added statistical information about the age, gender, and occupation of persons in the TikTalkCoref dataset in Appendix \ref{appendix:key information}. Moreover, we have added statistics of the celebrity data in Table \ref{tab:data basic statistics} and a comparison of the size of our dataset with existing multimodal coreference resolution datasets in Table \ref{tab:dataset_comparison}.

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 3:} \textit{Some issues in experiment design are not clear enough. For example, why take e2e-coref as a baseline for textual coreference resolution? Why not use all the 1,012 dialogues or the 674 dialogues without celebrities in the experiments?} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} 
% We would like to clarify the issues in our experimental design.

\textbf{• Utilization of e2e-coref:} We choose e2e-coref \cite{lee-etal-2017-endtoend} as the baseline model because it performs well in coreference resolution and is widely used. As a simple and effective end-to-end model, e2e-coref adapts well to our task through fine-tuning. Following \citet{goel-etal-2023-who}, we use e2e-coref as the baseline for textual coreference resolution. We have added the reason of using e2e-coref in Section \ref{sec:Experimental Settings}.

\textbf{• Leveraging non-celebrity for data augmentation:} To ensure data quality and domain adaptability, we focus on the celebrity domain. To fully utilize our annotated data and improve model performance, we incorporate 674 non-celebrity dialogues into the training of the text coreference resolution module. This approach is intended for data augmentation but also aimed to explore whether celebrity and non-celebrity data share similar linguistic features. We have added the explanation of leveraging non-celebrity in Section \ref{sec:Experimental Settings}.

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 4:} \textit{It would be better to include more existing multimodal coreference resolution models for comparison in the experiments.}

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} Due to language and data scale issues, we don't use existing multimodal coreference resolution models. For details, please refer to the \textbf{Response to Meta Reviewer}.

\vspace{1em}  % 调整段落间距
\section*{Response to Reviewer b4eS}
\textbf{Question 1:} \textit{Baselines do ``late fusion'', in that they do textual co-reference and entity tracking separately. To justify the label ``multimodal co-reference detection'', it seems that it would be better to explore if modalities can support each other.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} Following \citet{goel-etal-2023-who}, we adopt a ``late fusion'' approach in our baseline method, which can simplify model design and improve flexibility in handling modality-specific tasks. Considering the ``early fusion'' may enhance modal complementarity and robustness, we plan to explore this approach to improve cross-modal coreference alignment in future work.
% This approach can help us simplify the task, but we also realize that it fails to fully explore the potential of multimodal fusion in coreference detection. 

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 2:} \textit{Linking needs to happen via recognition of persons. It seems that a more interesting task would be co-reference and linking for phrasal NPs, not named entities.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} 
We primarily link images through names in the coreference chains. However, even when names are absent, our model can still link the image. If the chain includes both a name and an NP phrase, the model links through the name. If the chain only contains an NP phrase, the model links through the phrase. The linking accuracy depends on the clues the model extracts from the text and its understanding of the image. 

\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 3:} \textit{The explanation of ``TikTalkCoref performs better in capturing the complexity and diversity of multimodal information interaction in the real world'' is a fairly sweeping claim.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} 
% Our statement in the last version may have been lacking in consideration, as this is not a conclusion that can be drawn simply by example. Therefore, 
We have revised our statement to make it more rigorous in Section \ref{sec:Introduction} and Section \ref{sec:Related Work}.

\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 4:} \textit{The definition of ``cross-modal coreferential relationships'' is not clear enough.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} In our paper, ``textual co-reference relations'' and ``linking relations'' are referred to as ``cross-modal coreferential relationships,'' where text references and video regions co-refer to the same entity. This assumes that visual regions in the video correspond to entities mentioned in the text. We have added detailed explanation in Section \ref{sec:Introduction}.


\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 5:} \textit{What exactly were the criteria for exclusion mentioned in line 188?} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We filter high-quality data available for annotating coreference relationships through three criteria, as detailed in Section \ref{sec:Data Selection}:

(1) No privacy issues: Excludes content with personal identifying information or sensitive details.

(2) Clear video quality: Excludes videos with significant blurriness or noise, ensuring faces are identifiable.

(3) Dialogue mentions entities: Excludes dialogues that do not clearly mention person entities for coreference resolution.


\vspace{1em}  % 调整段落间距

\noindent \textbf{Question 6:} \textit{What are your criteria for knowing whether an entity is captured by the label ``celebrity'' (line 469)?} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We define a "celebrity" based on two criteria, as detailed in Section \ref{sec:Annotation Guidelines}:

(1) The person is regularly featured in public media and has a widely recognized public image.

(2) Based on common knowledge, annotators agree that the person is a ``celebrity''.

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 6:} \textit{``In this work, we focus on multimodal coreference resolution for celebreties'' (line 469) -- It seems this should come earlier than page 6.}

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have added the explanation of task domain in Abstract and Section \ref{sec:Introduction}.


\vspace{1em}  % 调整段落间距
\section*{Response to Reviewer wRGo}

\textbf{Question 1:} \textit{The new dataset has a small amount of data, which actually limits the scope of application of the constructed dataset.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have made our best efforts in the annotation process and have annotated 1,012 dialogues, which will advance research in Chinese multimodal coreference resolution. In the future, we will continue to expand the scale of the dataset. Please see the \textbf{Response to Meta Reviewer} for more details.

\vspace{1em}  % 调整段落间距
\noindent \textbf{Question 2:} \textit{Lack of explanation for the evaluation metrics.} 

\vspace{0.5em}  % 调整段落间距
\noindent \textbf{Our Response:} We have added an explanation of the evaluation metrics used in Appendix \ref{appendix:evaluation indicators}.

\vspace{1em}  % 调整段落间距
Best regards,

Anonymous ACL submission authors

